Testing Isomorphism of Boolean Functions over Finite Abelian Groups

Let $f$ and $g$ be Boolean functions over a finite Abelian group $\mathcal{G}$, where $g$ is fully known, and we have {\em query access} to $f$, that is, given any $x \in \mathcal{G}$ we can get the value $f(x)$. We study the tolerant isomorphism testing problem: given $\epsilon \geq 0$ and $\tau > 0$, we seek to determine, with minimal queries, whether there exists an automorphism $\sigma$ of $\mathcal{G}$ such that the fractional Hamming distance between $f \circ \sigma$ and $g$ is at most $\epsilon$, or whether for all automorphisms $\sigma$, the distance is at least $\epsilon + \tau$. We design an efficient tolerant testing algorithm for this problem, with query complexity $\mathrm{poly}\left( s, 1/\tau \right)$, where $s$ bounds the spectral norm of $g$. Additionally, we present an improved algorithm when $g$ is Fourier sparse. Our approach uses key concepts from Abelian group theory and Fourier analysis, including the annihilator of a subgroup, Pontryagin duality, and a pseudo inner-product for finite Abelian groups. We believe these techniques will find further applications in property testing.

==> Goldreich_Levin_generalized.tex <==
\section{Generalization of Goldreich-Levin Theorem}

Throughout this section, $\G$ denotes a finite Abelian group, hence $\G=\mathbb{Z}_{p_1^{n_1}} \times \cdots \times \mathbb{Z}_{p_T^{n_T}}$, where $p_i, i \in [T]$ are primes and not necessarily distinct. Let $n = \LCM \{p_1^{n_1}, \ldots, p_T^{n_T}\}$. 



\begin{algorithm}
\caption{Generalized Goldreich-Levin for $\G$}\label{algo:Goldreich_Levin_generalized}
\begin{algorithmic}
    \Statex \textbf{Input:} Given $\G$, a finite Abelian group, hence $\G=\mathbb{Z}_{p_1^{n_1}}\times \cdots \times \mathbb{Z}_{p_T^{n_T}}$, where $p_i$ are primes for all $i \in [T]$ and not necessarily distinct. A Boolean valued function $f:\G \to \{-1,+1\}$ and its characters contained in a single bucket $\mathcal{B}$.
    \Statex \textbf{Output:} Buckets $\mathcal{B}_\mathcal{S}$ with weight at least $\frac{\eta^2}{2}$ containing a single character $\chi_r$ such that $r\in \mathcal{S}$, where $\mathcal{S}\subseteq [T]$.

    \State \textbf{Initialize} bucket $\mathcal{B}$ with $|\G|$ many characters, where $|G|$ denotes the order of the group $G$.

    \State Split $\mathcal{B}$ into $p_1^{n_1}$ equal sized buckets $\mathcal{B}_0, \mathcal{B}_1, \ldots, \mathcal{B}_{p_1^{n_1}-1}$ in the first step.

    \State Find the weight of each $\mathcal{B}_i$, $i \in [2]$, where $\wt(\mathcal{B}_i) = \sum_{r \in \mathcal{B}_i} |\widehat{f}(\chi_r)|^2$. 

    \State If $\wt(\mathcal{B}_i) \leq \frac{\eta^2}{2}$, $i \in [2]$, discard $\mathcal{B}_i$. Otherwise, continue the process for each bucket.

    \State In the next step, split each bucket into $p_2^{n_2}$ many buckets, and continue the process in the same way.

    \State Stop when all the buckets contain at most one character.

    \State \textbf{Return} the buckets.
\end{algorithmic}
\end{algorithm}


Algorithm~\ref{algo:Goldreich_Levin_generalized} takes a Boolean valued function $f$ on $\G$ and a bucket $\mathcal{B}$ containing all its characters as input and outputs those buckets whose weight is $\geq \frac{\eta^2}{2}$, where $\mathcal{S}\subseteq [T]$. 
% Here $\mathcal{S} \subseteq [n]$ denotes those characters $\chi_r$, $r=(r_1, \ldots, r_n)$ such that $r_i\neq 0$ for $i \in \mathcal{S}$, and $0$ otherwise. 


In the first step, we divide the bucket $\mathcal{B}$ into $p_1^{n_1}$ buckets $\mathcal{B}_0, \ldots, \mathcal{B}_{p_1^{n_1}-1}$, where $\mathcal{B}_{i_1} = \{\chi_{(r_1, \ldots, r_T)} : r_{1}=i_1\}$, where $r_j \in \{0,\ldots,p_1^{n_1}-1\} \ \forall j \neq i_1$. We weigh the buckets and discard those with weight $\leq \frac{\eta^2}{2}$.
%\textcolor{blue}{need a description of ${i_1, \ldots, i_k}$ as well}
In the $k^{th}$ step, each surviving bucket is divided into $p_k^{n_k}$ buckets. Let us denote the buckets by $\mathcal{B}_{i_1, \ldots, i_k}$, where 
\begin{align*}
    \mathcal{B}_{i_1, \ldots, i_k} = \{\chi_{(r_1,\ldots, r_n)} : r_1= i_1, \ldots, r_k=i_k\},
\end{align*}
$r_j \in \{0,\ldots,p_j^{n_j}-1\} \ \forall j \neq i_1, \ldots, i_k$. 

The weight of a bucket $\mathcal{B}_{i_1, \ldots, i_k}$ is given by
\begin{align*}
    \wt \bigl( \mathcal{B}_{i_1, \ldots, i_k} \bigr) = \sum_{(r_1,\ldots,r_T) \in \G : r_1=i_1, \ldots, r_k=i_k} |\widehat{f}(\chi_{(r_1, \ldots, r_T)})|^2.
\end{align*}

Now let us look at the normal subgroup $H$ defined by 
\begin{align*}
    H= \{\gamma \in \G : \gamma \cdot e_1 =0, \ldots, \gamma\cdot e_k=0\},
\end{align*}
where $e_j$ is the element in $\G$ whose $j^{th}$ coordinate equals $1$ and the rest are $0$.

Observe that the bucket $\mathcal{B}_{i_1, \ldots, i_k}$ is the coset $\alpha+H$ of $H$, where $\alpha \cdot e_j = i_j$ for all $j \in [k]$. Let us denote this bucket by $\mathcal{B}_{\alpha+H}$.



\begin{lemma}
Let 
$\chi_{\alpha(C)}$ be the character in the bucket $C$ (with high probability). Algorithm~\ref{algo:Goldreich_Levin_generalized} does the following:
    \begin{enumerate}
        \item It does not discard any bucket $C$ with $|\widehat{f}(\chi_{\alpha(C)})| \geq \eta$.
        \item It discards any bucket $C$ with $|\widehat{f}(\chi_{\alpha(C)})| \leq \frac{\eta}{2}$.
    \end{enumerate}
\end{lemma}


\begin{proof}
\begin{description}
    \item[\textbf{Proof of part (1).}] $|\widehat{f}(\chi_{\alpha(C)})| \geq \eta \Rightarrow \Tilde{\wt_2}(C) \geq \eta^2 - \frac{\eta^2}{4} = \frac{3\eta^2}{4}$, which is $> \frac{\eta^2}{2}$. Hence the bucket $C$ is not discarded.

    \item[\textbf{Proof of part (2).}] When $|\widehat{f}(\chi_{\alpha(C)})| \leq \frac{\eta}{2}$, the estimated weight is either $\Tilde{\wt_2}(C) \leq \frac{\eta^2}{4}+\frac{\eta^2}{4} = \frac{\eta^2}{2}$, or $\Tilde{\wt_2}(C) = \frac{\eta^2}{4}-\frac{\eta^2}{4} =0$. Therefore, the bucket is discarded.
\end{description}
    
\end{proof}

% \begin{remark}
%     Since the group of characters $\widehat{\mathbb{Z}_{p^m}^n}$ of $\mathbb{Z}_{p^m}^n$, known as the Dual group of $\mathbb{Z}_{p^m}^n$, is isomorphic to $\mathbb{Z}_{p^m}^n$, so we can think of a character $\chi_r$ as an element $r$, $r \in \mathbb{Z}_{p^m}^n$.
% \end{remark}





Now, let us set the parameters $\epsilon$ and $\delta$ in \cref{eqn_wt_2_estimate}. Let us set $\epsilon=\frac{\eta}{2}$. Then, the weights of the buckets are estimated within $\pm \frac{\eta^2}{4}$, which implies that the buckets that we are not discarding have weight $\geq \frac{\eta^2}{4}$. Since the sum of the weights of the buckets cannot exceed $1$ by Parseval, the number of buckets we are not discarding cannot exceed $\frac{4}{\eta^2}$. Also, since in the $k^{th}$ step, a bucket is divided into $p_k^{n_k}$ buckets, a bucket is being divided at most $T$ times by the end of the loop. So the total number of loops the algorithm runs is equal to $\frac{4T}{\eta^2}$. Therefore, the total number of times the algorithm weighs is at most $\frac{4T}{\eta^2} \times \max_{j \in [T]} \{p_j^{n_j}\}$. 

Now, observe that we want to estimate the weight of all the buckets with high probability, say $\frac{99}{100}$, for which we need $4 \ln(\frac{4}{\delta})/\epsilon^2 \times\frac{4T}{\eta^2} \times \max_{j \in [T]} \{p_j^{n_j}\} = 64 \ln(\frac{4T}{\delta})/(\eta^4) \times \max_{j \in [T]} \{p_j^{n_j}\}$ many samples by Lemma~\ref{lemma_wt_estimate_new}. Also, the total error probability of weighing is equal to $\delta \times \frac{4T}{\eta^2} \times \max_{j \in [T]} \{p_j^{n_j}\}$ by union bound. Therefore, setting $\delta = \frac{\eta^2}{400T \times \max_{j \in [T]} \{p_j^{n_j}\}}$, we have the error probability to be $\leq \frac{1}{100}$. Hence, the total number of samples required $= 64 \ln(\frac{1600T^2 \max_{j \in [T]} \{p_j^{n_j}\}}{\eta^2})/(\eta^4) \times \max_{j \in [T]} \{p_j^{n_j}\}$, which is $\poly(\frac{1}{\eta}, T)$, since we are considering $p_j^{n_j}, j \in [T]$ to be constants.


